READ: Reliability-Enhanced Accelerator Dataflow Optimization using Critical Input Pattern Reduction

With the rapid advancements of deep learning in recent years, hardware accelerators are continuously deployed in more and more safety-critical applications such as autonomous driving and robotics. While the accelerators are usually fabricated with advanced technology nodes for high performance and energy efficiency, they are also more prone to timing errors under process, voltage, temperature, and aging (PVTA) variations. By revisiting the physical sources of timing errors, we show that most of the timing errors in the accelerator are caused by a specific subset of input patterns, defined as critical input patterns. To improve the timing error resilience of the accelerator, in this paper, we propose READ, a reliability-enhanced accelerator dataflow optimization technique that can effectively reduce timing errors. READ reduces the occurrence of critical input patterns by exploring the optimal computing sequence when mapping a trained deep neural network to accelerators. READ only changes the order of multiply-accumulate operations in a convolution, which introduces negligible hardware overhead and no impact on accuracy. The experimental results on VGG and ResNet demonstrate on average 7.8X timing error rate (TER) reduction and up to 37.9X TER reduction for certain layers. The results also show that READ enables the accelerator to maintain accuracy over a wide range of PVTA variations, making it a promising approach for robust deep-learning design

==> doc/5-related-works.tex <==
\section{Related Work}
\label{sec:related-work}
To improve the timing error resilience of accelerators, a number of approaches from model-layer to circuit-layer have been proposed.
The model-layer techniques utilize the NN's inherent redundancy and tolerance for errors, 
and common methods include sensitivity analysis, fault/noise-tolerant training, and model architecture design. 
Choi et al. proposed to evaluate filter/channel-level weight sensitivities and assign sensitive weights to robust PE to improve error resilience~\cite{sensitivity_analysis_dnn}.
Schorn et al. propose a training strategy to adjust neuron sensitivities~\cite{resilience-optimization-schorn}, 
which argues that achieving a homogeneous resilience distribution can help DNN robustness.
Liu et al. proposed to use error-correcting output codes (ECOC) to tolerate variations and faults~\cite{ECOC-dac}.
Our work is a post-training optimization technique, so the model-layer techniques are orthogonal to our work.

Circuit-layer techniques usually utilize timing error detection (using Razor flip-flops~\cite{razor}, for instance) and correction approaches.
Zhang et al. introduced a new timing speculation methodology for accelerators, 
in which the MAC unit encountering a timing error, will steal an execution cycle from its downstream MAC to recover the correct value~\cite{thundervolt}.
Gundi et al. further improved the correction scheme~\cite{EFFORT-dac}. 
Whatmough et al. proposed a scheme that utilizes lightweight Razor flip-flops and circuit-layer timing borrowing to tolerate the timing errors~\cite{DNN_Engine}.
However, our work is the first one that exploits the impact of dataflow on timing errors, and does not need any hardware modification in the computing array.
Moreover, the proposed optimization algorithm can be also deployed on the timing speculation accelerator to reduce the toggle rate of TEDC modules, 
and enable more aggressive overclocking or voltage scaling for higher energy efficiency.


==> texlib/acm_setting.tex <==
% =============================================================
%            settign for ACM format paper
%
%   Author      : Bei Yu
%   Last Update : 12/2014
% =============================================================

\settopmatter{printacmref=false}          % no ACM Reference Format
\fancyhead{}                              % no header

% ==== page margin settings
\geometry{twoside=true, head=13pt,
	paperwidth=8.5in, paperheight=11in,
	includeheadfoot, columnsep=2pc,
	top=45pt, bottom=55pt, 
    left=45pt, right=45pt, 
    %inner=54pt, outer=54pt,
	marginparwidth=2pc,heightrounded
}%
\iffalse
\textfloatsep          = 12pt plus 1pt minus 7pt            % set space between figure and text
\floatsep              = 5pt plus 1pt minus 7pt
\fi
%\intextsep             = 0pt plus 1pt minus 7pt           % set space above and below the texts
%\dbltextfloatsep       = 0pt plus 1pt minus 7pt
%\dblfloatsep           = 0pt plus 1pt minus 7pt
%\abovedisplayskip      = 0pt plus 1pt minus 7pt           % set space around equations
%\belowdisplayskip      = 0pt plus 1pt minus 7pt
%\abovedisplayshortskip = 0pt plus 1pt minus 7pt
%\belowdisplayshortskip = 0pt plus 1pt minus 7pt

% ==== Packages
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{comment}
\usepackage[subrefformat=parens,labelformat=parens]{subfig}
\captionsetup[subfigure]{labelformat=simple}               % avoid "double brackets" in sub-figure caption
\renewcommand\thesubfigure{(\alph{subfigure})}             % "Fig.~1b"-->"Fig.1(b)"
\usepackage{bm}
\usepackage{multirow}
\usepackage{threeparttable,booktabs}
\usepackage{tikz}
\usepackage{balance}
\usepackage{courier}                                       % courier font, used in \texttt
\usepackage{cleveref}                                      % smart citation
%\usepackage[mathcal]{eucal}
%\usepackage[]{algpseudocode}                               % algorithm package
\usepackage[noend]{algpseudocode}
\algrenewcommand\textproc{\texttt}
\makeatletter\let\float@addtolists\relax\makeatother
\usepackage{algorithm}
\renewcommand{\algorithmicrequire}{\textbf{Input:} }       % Use Input in the format of Algorithm
\renewcommand{\algorithmicensure} {\textbf{Output:}}       % Use Output in the format of Algorithm
\usepackage{filecontents}                                  % support to pgfplots
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\pgfplotsset{compat=newest}
\usepackage{siunitx}
\sisetup{product-units = single}
% ==== Local new commands
%\newcommand{\calH}{\mathcal{H}}
%\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
%\newcommand{\calP}{\mathcal{P}}
%\newcommand{\calV}{\mathcal{V}}
%\newcommand{\calS}{\mathcal{S}}
%\newcommand{\calD}{\mathcal{D}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\renewcommand{\vec}[1]{\boldsymbol{#1}} 
%\newcommand{\m}[1]{\mathbf{#1}}
%\newcommand{\mx}{\m{x}}
%\newcommand{\my}{\m{y}}
%\newcommand{\mz}{\m{z}}
\DeclareMathOperator*{\argmin}{argmin}

\theoremstyle{plain}
\newtheorem{mytheorem}{\textbf{Theorem}}
\newtheorem{mylemma}{\textbf{Lemma}}
\newtheorem{myclaim}{\textbf{Claim}}

\theoremstyle{definition}
\newtheorem{mydefinition}{\textbf{Definition}}
\newtheorem{myproblem}{\textbf{Problem}}



% ==== spacing control on caption
\usepackage[skip=1pt]{caption}            % set space between figure and caption
\setlength{\belowcaptionskip}{-1.0mm}
\captionsetup[table]{aboveskip=5pt}       % reduce space around table caption
\captionsetup[table]{belowskip=2pt}


==> texlib/poster_setting.tex <==
% ============================================================
%             Beamer poster setting file
%
%   Author      : Bei Yu
%   last Update : 06/2014
% ============================================================

% additional settings
\setbeamerfont{itemize}{size=\normalsize}
\setbeamerfont{itemize/enumerate body}{size=\normalsize}
\setbeamerfont{itemize/enumerate subbody}{size=\normalsize}


% block width setting
\newenvironment<>{varblock}[2][\textwidth]{%
  \setlength{\textwidth}{#1}
  \setbeamercolor{block title}{fg=white,bg=blue!20!green}
  %\setbeamercolor{block body}{fg=black,bg=olive!50}
  \setbeamercolor{block body}{fg=black,bg=blue!10}
  \begin{actionenv}#3%
  \def\insertblocktitle{#2}%
  \par%
  \usebeamertemplate{block begin}}
  {
    \par%
    \usebeamertemplate{block end}%
    \end{actionenv}
  }


% abbreviations
\usepackage{xspace}
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{{e.g}\onedot} \def\Eg{{E.g}\onedot}
\def\ie{{i.e}\onedot} \def\Ie{{I.e}\onedot}
\def\cf{{c.f}\onedot} \def\Cf{{C.f}\onedot}
\def\etc{{etc}\onedot}
\def\vs{{vs}\onedot}
\def\wrt{w.r.t\onedot}
\def\dof{d.o.f\onedot}
\def\etal{{et al}\onedot}
\makeatother


% === including packages
\usepackage{bm}
\usepackage{xcolor}
\usepackage{colortbl}
\usepackage{times}
\usepackage{amsmath,amsthm, amssymb, latexsym}
\usepackage{exscale}
\usepackage{subfigure}
\usepackage{multirow}
\usepackage{comment}
\usepackage{booktabs, array}
\usepackage[english]{babel}
\usepackage[latin1]{inputenc}
\usepackage[orientation=landscape,size=custom,width=200,height=230,scale=1.9]{beamerposter}
\listfiles

% =====  algorithm setting
%\usepackage[noend]{algpseudocode}
\usepackage{algpseudocode}
\usepackage{algorithm}
%\renewcommand{\algorithmicrequire}{\textbf{Input:}}  % Use Input in the format of Algorithm
%\renewcommand{\algorithmicensure}{\textbf{Output:}} % Use Output in the format of Algorithm

% ==== Log
%
%  05/2014: preliminary results show that pgf library is NOT good for poster
%


